Beam test results of 25 $\mu$m and 35 $\mu$m thick FBK UFSD]{Beam test results of 25 $\mu$m and 35 $\mu$m thick FBK ultra fast silicon detectors

This paper presents the measurements on first very thin Ultra Fast Silicon Detectors (UFSDs) produced by Fondazione Bruno Kessler; the data have been collected in a beam test setup at the CERN PS, using beam with a momentum of 12 GeV/c. UFSDs with a nominal thickness of 25 $\mu$m and 35 $\mu$m and an area of 1 $\times$ 1 $\text{mm}^2$ have been considered, together with an additional HPK 50-$\mu$m thick sensor, taken as reference. Their timing performances have been studied as a function of the applied voltage and gain. A time resolution of about 25 ps and of 22 ps at a voltage of 120 V and 240 V has been obtained for the 25 and 35 $\mu$m thick UFSDs, respectively.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


